Exciton Binding Energies in 2D Materials: Insights from Braneworld Physics

In the present work, we introduce a new interpretation of exciton binding energies in two-dimensional (2D) materials using concepts from brane physics. We adapt the Dvali-Gabadadze-Porrati-Shifman mechanism to a (2+1)-dimensional brane in a (3+1)-D spacetime, deriving an effective electromagnetic potential on the brane. Using this potential, we develop a hydrogenic model for exciton binding energies in 2D materials, applying it to s-type excitons and comparing theoretical predictions with experimental results on WS$_{2}$ monolayers. This interdisciplinary approach bridges high-energy and condensed matter physics, offering a new didactic representation of excitons in low-dimensional systems.

==> bibliography_save <==

@article{hichri_exciton_nodate,
	title = {Exciton, trion and localized exciton in monolayer Tungsten Disulfide},
	author = {Hichri, Aïda and Amara, Imen Ben and Ayari, Sabrine and Jaziri, Sihem},
	langid = {english},
	file = {Hichri et al. - Exciton, trion and localized exciton in monolayer .pdf:C\:\\Users\\ahonet\\Zotero\\storage\\JLC7MWGP\\Hichri et al. - Exciton, trion and localized exciton in monolayer .pdf:application/pdf},
}

@article{geng_recent_2018,
	title = {Recent Advances in Growth of Novel 2D Materials: Beyond Graphene and Transition Metal Dichalcogenides},
	volume = {30},
	issn = {0935-9648, 1521-4095},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/adma.201800865},
	doi = {10.1002/adma.201800865},
	shorttitle = {Recent Advances in Growth of Novel 2D Materials},
	pages = {1800865},
	number = {45},
	journaltitle = {Advanced Materials},
	shortjournal = {Adv. Mater.},
	author = {Geng, Dechao and Yang, Hui Ying},
	urldate = {2023-08-31},
	date = {2018-11},
	langid = {english},
	file = {Geng and Yang - 2018 - Recent Advances in Growth of Novel 2D Materials B.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\G3R6TWAV\\Geng and Yang - 2018 - Recent Advances in Growth of Novel 2D Materials B.pdf:application/pdf},
}

@article{hichri_exciton_2017,
	title = {Exciton center-of-mass localization and dielectric environment effect in monolayer {WS}2},
	volume = {121},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/121/23/235702/143726/Exciton-center-of-mass-localization-and-dielectric},
	doi = {10.1063/1.4984790},
	abstract = {The ultrathin transition metal dichalcogenides ({TMDs}) have emerged as promising materials for various applications using two dimensional semiconductors. They have attracted increasing attention due to their unique optical properties originate from neutral and charged excitons. In this paper, we study the strong localization of exciton center-of-mass motion within random potential fluctuations caused by the monolayer defects. Here, we report negatively charged exciton formation in monolayer {TMDs}, notably tungsten disulfide {WS}2. Our theory is based on an effective mass model of neutral and charged excitons, parameterized by ab-initio calculations. Taking into the account the strong correlation between the monolayer {WS}2 and the surrounding dielectric environment, our theoretical results are in good agreement with one-photon photoluminescence ({PL}) and reflectivity measurements. We also show that the exciton state with p-symmetry, experimentally observed by two-photon {PL} emission, is energetically below the 2s-state. We use the equilibrium mass action law, to quantify the relative weight of exciton and trion {PL}. We show that exciton and trion emission can be tuned and controlled by external parameters like temperature, pumping, and injection electrons. Finally, in comparison with experimental measurements, we show that exciton emission in monolayer tungsten dichalcogenides is substantially reduced. This feature suggests that free exciton can be trapped in disordered potential wells to form a localized exciton and therefore offers a route toward novel optical properties.},
	pages = {235702},
	number = {23},
	journaltitle = {Journal of Applied Physics},
	author = {Hichri, Aïda and Ben Amara, Imen and Ayari, Sabrine and Jaziri, Sihem},
	urldate = {2023-08-31},
	date = {2017-06-21},
	langid = {english},
	file = {Hichri et al. - 2017 - Exciton center-of-mass localization and dielectric.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\YLR29YXG\\Hichri et al. - 2017 - Exciton center-of-mass localization and dielectric.pdf:application/pdf},
}

@article{yang_analytic_1991,
	title = {Analytic solution of a two-dimensional hydrogen atom. I. Nonrelativistic theory},
	volume = {43},
	issn = {1050-2947, 1094-1622},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.43.1186},
	doi = {10.1103/PhysRevA.43.1186},
	pages = {1186--1196},
	number = {3},
	journaltitle = {Physical Review A},
	shortjournal = {Phys. Rev. A},
	author = {Yang, X. L. and Guo, S. H. and Chan, F. T. and Wong, K. W. and Ching, W. Y.},
	urldate = {2023-08-31},
	date = {1991-02-01},
	langid = {english},
	file = {Yang et al. - 1991 - Analytic solution of a two-dimensional hydrogen at.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\MK67Z7VW\\Yang et al. - 1991 - Analytic solution of a two-dimensional hydrogen at.pdf:application/pdf},
}

@article{cudazzo_dielectric_2011,
	title = {Dielectric screening in two-dimensional insulators: Implications for excitonic and impurity states in graphane},
	volume = {84},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.84.085406},
	doi = {10.1103/PhysRevB.84.085406},
	shorttitle = {Dielectric screening in two-dimensional insulators},
	pages = {085406},
	number = {8},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Cudazzo, Pierluigi and Tokatly, Ilya V. and Rubio, Angel},
	urldate = {2023-08-31},
	date = {2011-08-19},
	langid = {english},
	file = {Cudazzo et al. - 2011 - Dielectric screening in two-dimensional insulators.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\XRP44MIV\\Cudazzo et al. - 2011 - Dielectric screening in two-dimensional insulators.pdf:application/pdf},
}

@article{ramasubramaniam_large_2012,
	title = {Large excitonic effects in monolayers of molybdenum and tungsten dichalcogenides},
	volume = {86},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.86.115409},
	doi = {10.1103/PhysRevB.86.115409},
	pages = {115409},
	number = {11},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Ramasubramaniam, Ashwin},
	urldate = {2023-08-31},
	date = {2012-09-06},
	langid = {english},
	file = {Ramasubramaniam - 2012 - Large excitonic effects in monolayers of molybdenu.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\G5IZDBH6\\Ramasubramaniam - 2012 - Large excitonic effects in monolayers of molybdenu.pdf:application/pdf},
}

@article{horzum_phonon_2013,
	title = {Phonon softening and direct to indirect band gap crossover in strained single-layer {MoSe} 2},
	volume = {87},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.87.125415},
	doi = {10.1103/PhysRevB.87.125415},
	pages = {125415},
	number = {12},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Horzum, S. and Sahin, H. and Cahangirov, S. and Cudazzo, P. and Rubio, A. and Serin, T. and Peeters, F. M.},
	urldate = {2023-08-31},
	date = {2013-03-14},
	langid = {english},
	file = {Horzum et al. - 2013 - Phonon softening and direct to indirect band gap c.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\R76RDR9L\\Horzum et al. - 2013 - Phonon softening and direct to indirect band gap c.pdf:application/pdf},
}

@article{shi_quasiparticle_2013,
	title = {Quasiparticle band structures and optical properties of strained monolayer {MoS} 2 and {WS} 2},
	volume = {87},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.87.155304},
	doi = {10.1103/PhysRevB.87.155304},
	pages = {155304},
	number = {15},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Shi, Hongliang and Pan, Hui and Zhang, Yong-Wei and Yakobson, Boris I.},
	urldate = {2023-08-31},
	date = {2013-04-09},
	langid = {english},
	file = {Shi et al. - 2013 - Quasiparticle band structures and optical properti.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\QGPEKTIB\\Shi et al. - 2013 - Quasiparticle band structures and optical properti.pdf:application/pdf},
}

@article{berkelbach_theory_2013,
	title = {Theory of neutral and charged excitons in monolayer transition metal dichalcogenides},
	volume = {88},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.88.045318},
	doi = {10.1103/PhysRevB.88.045318},
	pages = {045318},
	number = {4},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Berkelbach, Timothy C. and Hybertsen, Mark S. and Reichman, David R.},
	urldate = {2023-08-31},
	date = {2013-07-25},
	langid = {english},
	file = {Berkelbach et al. - 2013 - Theory of neutral and charged excitons in monolaye.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\TXTDCEUI\\Berkelbach et al. - 2013 - Theory of neutral and charged excitons in monolaye.pdf:application/pdf},
}

@article{chernikov_exciton_2014,
	title = {Exciton Binding Energy and Nonhydrogenic Rydberg Series in Monolayer {WS} 2},
	volume = {113},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.113.076802},
	doi = {10.1103/PhysRevLett.113.076802},
	pages = {076802},
	number = {7},
	journaltitle = {Physical Review Letters},
	shortjournal = {Phys. Rev. Lett.},
	author = {Chernikov, Alexey and Berkelbach, Timothy C. and Hill, Heather M. and Rigosi, Albert and Li, Yilei and Aslan, Burak and Reichman, David R. and Hybertsen, Mark S. and Heinz, Tony F.},
	urldate = {2023-08-31},
	date = {2014-08-13},
	langid = {english},
	file = {Chernikov et al. - 2014 - Exciton Binding Energy and Nonhydrogenic Rydberg S.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\MLD86MT8\\Chernikov et al. - 2014 - Exciton Binding Energy and Nonhydrogenic Rydberg S.pdf:application/pdf},
}

@article{novoselov_electric_2004,
	title = {Electric Field Effect in Atomically Thin Carbon Films},
	volume = {306},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1102896},
	doi = {10.1126/science.1102896},
	abstract = {We describe monocrystalline graphitic films, which are a few atoms thick but are nonetheless stable under ambient conditions, metallic, and of remarkably high quality. The films are found to be a two-dimensional semimetal with a tiny overlap between valence and conductance bands, and they exhibit a strong ambipolar electric field effect such that electrons and holes in concentrations up to 10
              13
              per square centimeter and with room-temperature mobilities of ∼10,000 square centimeters per volt-second can be induced by applying gate voltage.},
	pages = {666--669},
	number = {5696},
	journaltitle = {Science},
	shortjournal = {Science},
	author = {Novoselov, K. S. and Geim, A. K. and Morozov, S. V. and Jiang, D. and Zhang, Y. and Dubonos, S. V. and Grigorieva, I. V. and Firsov, A. A.},
	urldate = {2023-08-31},
	date = {2004-10-22},
	langid = {english},
	file = {Novoselov et al. - 2004 - Electric Field Effect in Atomically Thin Carbon Fi.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\PNL3495N\\Novoselov et al. - 2004 - Electric Field Effect in Atomically Thin Carbon Fi.pdf:application/pdf},
}

@article{chernikov_supplemental_nodate,
	title = {Supplemental Material Non-hydrogenic Rydberg Series and Exciton Binding Energy in Monolayer {WS}2},
	author = {Chernikov, Alexey and Berkelbach, Timothy C and Hill, Heather M and Rigosi, Albert and Li, Yilei and Aslan, Özgur B and Reichman, David R and Hybertsen, Mark S and Heinz, Tony F},
	langid = {english},
	file = {Chernikov et al. - Supplemental Material Non-hydrogenic Rydberg Serie.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\76MGQU9K\\Chernikov et al. - Supplemental Material Non-hydrogenic Rydberg Serie.pdf:application/pdf},
}

@article{van_tuan_coulomb_2018,
	title = {Coulomb interaction in monolayer transition-metal dichalcogenides},
	volume = {98},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.98.125308},
	doi = {10.1103/PhysRevB.98.125308},
	pages = {125308},
	number = {12},
	journaltitle = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Van Tuan, Dinh and Yang, Min and Dery, Hanan},
	urldate = {2023-08-31},
	date = {2018-09-27},
	langid = {english},
	file = {Van Tuan et al. - 2018 - Coulomb interaction in monolayer transition-metal .pdf:C\:\\Users\\ahonet\\Zotero\\storage\\857MWUFP\\Van Tuan et al. - 2018 - Coulomb interaction in monolayer transition-metal .pdf:application/pdf},
}

@misc{rytova_screened_2020,
	title = {Screened potential of a point charge in a thin film},
	url = {http://arxiv.org/abs/1806.00976},
	abstract = {The potential of a point charge in a thin semiconducting film with the thickness below the de Broglie wavelength of the free charge carriers is calculated with and without the screening.},
	number = {{arXiv}:1806.00976},
	publisher = {{arXiv}},
	author = {Rytova, Natalia S.},
	urldate = {2023-08-31},
	date = {2020-09-01},
	langid = {english},
	eprinttype = {arxiv},
	eprint = {1806.00976 [cond-mat]},
	keywords = {Condensed Matter - Mesoscale and Nanoscale Physics},
	file = {Rytova - 2020 - Screened potential of a point charge in a thin fil.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\9C87F92C\\Rytova - 2020 - Screened potential of a point charge in a thin fil.pdf:application/pdf},
}

@article{goryca_revealing_2019,
	title = {Revealing exciton masses and dielectric properties of monolayer semiconductors with high magnetic fields},
	volume = {10},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-019-12180-y},
	doi = {10.1038/s41467-019-12180-y},
	abstract = {Abstract
            
              In semiconductor physics, many essential optoelectronic material parameters can be experimentally revealed via optical spectroscopy in sufficiently large magnetic fields. For monolayer transition-metal dichalcogenide semiconductors, this field scale is substantial—tens of teslas or more—due to heavy carrier masses and huge exciton binding energies. Here we report absorption spectroscopy of monolayer
              
                
                  \$\$\{\{{\textbackslash}rm\{{MoS}\}\}\}\_\{2\},\{\{{\textbackslash}rm\{{MoSe}\}\}\}\_\{2\},\{\{{\textbackslash}rm\{{MoTe}\}\}\}\_\{2\}\$\$
                  
                    
                      
                        {MoS}
                      
                      
                        2
                      
                    
                    ,
                    
                      
                        {MoSe}
                      
                      
                        2
                      
                    
                    ,
                    
                      
                        {MoTe}
                      
                      
                        2
                      
                    
                  
                
              
              , and
              
                
                  \$\$\{\{{\textbackslash}rm\{{WS}\}\}\}\_\{2\}\$\$
                  
                    
                      
                        {WS}
                      
                      
                        2
                      
                    
                  
                
              
              in very high magnetic fields to 91 T. We follow the diamagnetic shifts and valley Zeeman splittings of not only the exciton’s
              
                
                  \$\$1s\$\$
                  
                    1
                    s
                  
                
              
              ground state but also its excited
              
                
                  \$\$2s,3s,{\textbackslash}ldots ,ns\$\$
                  
                    2
                    s
                    ,
                    3
                    s
                    ,
                    …
                    ,
                    n
                    s
                  
                
              
              Rydberg states. This provides a direct experimental measure of the effective (reduced) exciton masses and dielectric properties. Exciton binding energies, exciton radii, and free-particle bandgaps are also determined. The measured exciton masses are heavier than theoretically predicted, especially for Mo-based monolayers. These results provide essential and quantitative parameters for the rational design of opto-electronic van der Waals heterostructures incorporating 2D semiconductors.},
	pages = {4172},
	number = {1},
	journaltitle = {Nature Communications},
	shortjournal = {Nat Commun},
	author = {Goryca, M. and Li, J. and Stier, A. V. and Taniguchi, T. and Watanabe, K. and Courtade, E. and Shree, S. and Robert, C. and Urbaszek, B. and Marie, X. and Crooker, S. A.},
	urldate = {2023-08-31},
	date = {2019-09-13},
	langid = {english},
	file = {Goryca et al. - 2019 - Revealing exciton masses and dielectric properties.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\U2FYXNPC\\Goryca et al. - 2019 - Revealing exciton masses and dielectric properties.pdf:application/pdf},
}

@article{mohammadzadeh_excitonic_2013,
	title = {Excitonic effects of bilayer graphene: A simple approach},
	volume = {124},
	issn = {00304026},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0030402613006153},
	doi = {10.1016/j.ijleo.2013.04.083},
	shorttitle = {Excitonic effects of bilayer graphene},
	pages = {6126--6131},
	number = {23},
	journaltitle = {Optik},
	shortjournal = {Optik},
	author = {Mohammadzadeh, L. and Shojaei, S. and Ahmadi, E. and Asgari, A.},
	urldate = {2023-08-31},
	date = {2013-12},
	langid = {english},
	file = {Mohammadzadeh et al. - 2013 - Excitonic effects of bilayer graphene A simple ap.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\9XC59ISH\\Mohammadzadeh et al. - 2013 - Excitonic effects of bilayer graphene A simple ap.pdf:application/pdf},
}

@article{dvali_4d_2000,
	title = {4D gravity on a brane in 5D Minkowski space},
	volume = {485},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0370269300006699},
	doi = {10.1016/S0370-2693(00)00669-9},
	abstract = {We suggest a mechanism by which four-dimensional Newtonian gravity emerges on a 3-brane in 5D Minkowski space with an infinite size extra dimension. The worldvolume theory gives rise to the correct 4D potential at short distances whereas at large distances the potential is that of a 5D theory. We discuss some phenomenological issues in this framework. q 2000 Elsevier Science B.V. All rights reserved.},
	pages = {208--214},
	number = {1},
	journaltitle = {Physics Letters B},
	shortjournal = {Physics Letters B},
	author = {Dvali, Gia and Gabadadze, Gregory and Porrati, Massimo},
	urldate = {2023-08-31},
	date = {2000-07},
	langid = {english},
	file = {Dvali et al. - 2000 - 4D gravity on a brane in 5D Minkowski space.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\XSIDSML5\\Dvali et al. - 2000 - 4D gravity on a brane in 5D Minkowski space.pdf:application/pdf},
}

@article{dvali_quasilocalized_2001,
	title = {(Quasi)localized gauge field on a brane: dissipating cosmic radiation to extra dimensions?},
	volume = {497},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0370269300013290},
	doi = {10.1016/S0370-2693(00)01329-0},
	shorttitle = {(Quasi)localized gauge field on a brane},
	abstract = {We propose a mechanism ensuring (quasi)localization of massless gauge ﬁelds on a brane. The mechanism does not rely on {BPS} properties of the brane and can be realized in any theory where charged particles are conﬁned to the world-volume. The localized matter ﬂuctuations induce a gauge kinetic term on the brane. At short distances the resulting propagator for the gauge ﬁeld is identical to the four-dimensional propagator. The gauge theory on the brane is effectively four-dimensional at short distances; it becomes higher-dimensional on very large (cosmic) scales. The brane-bulk system exhibits the phenomenon of “infrared transparency”. As a result, only very low frequency modes can escape into extra dimensions. In this framework the large wavelength cosmic radiation can dissipate in extra space at a rate that may be observable, in principle. We brieﬂy discuss some astrophysical consequences of this scenario.},
	pages = {271--280},
	number = {3},
	journaltitle = {Physics Letters B},
	shortjournal = {Physics Letters B},
	author = {Dvali, Gia and Gabadadze, Gregory and Shifman, M.},
	urldate = {2023-08-31},
	date = {2001-01},
	langid = {english},
	file = {Dvali et al. - 2001 - (Quasi)localized gauge field on a brane dissipati.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\9XU9VD8Y\\Dvali et al. - 2001 - (Quasi)localized gauge field on a brane dissipati.pdf:application/pdf},
}


==> references_s <==

@article{hichri_exciton_2016,
	title = {Exciton, trion and localized exciton in monolayer Tungsten Disulfide},
	rights = {{arXiv}.org perpetual, non-exclusive license},
	url = {https://arxiv.org/abs/1609.05634},
	doi = {10.48550/ARXIV.1609.05634},
	author = {Hichri, Aïda and Amara, Imen Ben and Ayari, Sabrine and Jaziri, Sihem},
	urldate = {2023-09-01},
	year = {2016},
	note = {Publisher: {arXiv}
Version Number: 1},
}

@article{geng_recent_2018,
	title = {Recent Advances in Growth of Novel 2{D} Materials: Beyond Graphene and Transition Metal Dichalcogenides},
	volume = {30},
	issn = {0935-9648, 1521-4095},
	doi = {10.1002/adma.201800865},
	shorttitle = {Recent Advances in Growth of Novel 2D Materials},
	pages = {1800865},
	number = {45},
	journal = {Adv. Mater.},
	author = {Geng, Dechao and Yang, Hui Ying},
	year = {2018},
	langid = {english},
}

@article{hichri_exciton_2017,
	title = {Exciton center-of-mass localization and dielectric environment effect in monolayer {WS}{$_\mathrm{2}$}},
	volume = {121},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/121/23/235702/143726/Exciton-center-of-mass-localization-and-dielectric},
	doi = {10.1063/1.4984790},
	pages = {235702},
	number = {23},
	journal = {Journal of Applied Physics},
	author = {Hichri, Aïda and Ben Amara, Imen and Ayari, Sabrine and Jaziri, Sihem},
	year = {2017},
	langid = {english},
}

@article{yang_analytic_1991,
	title = {Analytic solution of a two-dimensional hydrogen atom. {I}. {N}onrelativistic theory},
	volume = {43},
	issn = {1050-2947, 1094-1622},
	url = {https://link.aps.org/doi/10.1103/PhysRevA.43.1186},
	doi = {10.1103/PhysRevA.43.1186},
	pages = {1186--1196},
	number = {3},
	journal = {Physical Review A},
	shortjournal = {Phys. Rev. A},
	author = {Yang, X. L. and Guo, S. H. and Chan, F. T. and Wong, K. W. and Ching, W. Y.},
	urldate = {2023-08-31},
	date = {1991-02-01},
	langid = {english},
	file = {Yang et al. - 1991 - Analytic solution of a two-dimensional hydrogen at.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\MK67Z7VW\\Yang et al. - 1991 - Analytic solution of a two-dimensional hydrogen at.pdf:application/pdf},
}

@article{cudazzo_dielectric_2011,
	title = {Dielectric screening in two-dimensional insulators: Implications for excitonic and impurity states in graphane},
	volume = {84},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.84.085406},
	doi = {10.1103/PhysRevB.84.085406},
	shorttitle = {Dielectric screening in two-dimensional insulators},
	pages = {085406},
	number = {8},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Cudazzo, Pierluigi and Tokatly, Ilya V. and Rubio, Angel},
	urldate = {2023-08-31},
	date = {2011-08-19},
	langid = {english},
	file = {Cudazzo et al. - 2011 - Dielectric screening in two-dimensional insulators.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\XRP44MIV\\Cudazzo et al. - 2011 - Dielectric screening in two-dimensional insulators.pdf:application/pdf},
}

@article{ramasubramaniam_large_2012,
	title = {Large excitonic effects in monolayers of molybdenum and tungsten dichalcogenides},
	volume = {86},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.86.115409},
	doi = {10.1103/PhysRevB.86.115409},
	pages = {115409},
	number = {11},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Ramasubramaniam, Ashwin},
	urldate = {2023-08-31},
	date = {2012-09-06},
	langid = {english},
	file = {Ramasubramaniam - 2012 - Large excitonic effects in monolayers of molybdenu.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\G5IZDBH6\\Ramasubramaniam - 2012 - Large excitonic effects in monolayers of molybdenu.pdf:application/pdf},
}

@article{horzum_phonon_2013,
	title = {Phonon softening and direct to indirect band gap crossover in strained single-layer {MoSe} 2},
	volume = {87},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.87.125415},
	doi = {10.1103/PhysRevB.87.125415},
	pages = {125415},
	number = {12},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Horzum, S. and Sahin, H. and Cahangirov, S. and Cudazzo, P. and Rubio, A. and Serin, T. and Peeters, F. M.},
	urldate = {2023-08-31},
	date = {2013-03-14},
	langid = {english},
	file = {Horzum et al. - 2013 - Phonon softening and direct to indirect band gap c.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\R76RDR9L\\Horzum et al. - 2013 - Phonon softening and direct to indirect band gap c.pdf:application/pdf},
}

@article{shi_quasiparticle_2013,
	title = {Quasiparticle band structures and optical properties of strained monolayer {MoS}{$_\mathrm{2}$} and {WS}{$_\mathrm{2}$}},
	volume = {87},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.87.155304},
	doi = {10.1103/PhysRevB.87.155304},
	pages = {155304},
	number = {15},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Shi, Hongliang and Pan, Hui and Zhang, Yong-Wei and Yakobson, Boris I.},
	urldate = {2023-08-31},
	year = {2013},
	langid = {english}
}

@article{berkelbach_theory_2013,
	title = {Theory of neutral and charged excitons in monolayer transition metal dichalcogenides},
	volume = {88},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.88.045318},
	doi = {10.1103/PhysRevB.88.045318},
	pages = {045318},
	number = {4},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Berkelbach, Timothy C. and Hybertsen, Mark S. and Reichman, David R.},
	urldate = {2023-08-31},
	date = {2013-07-25},
	langid = {english},
	file = {Berkelbach et al. - 2013 - Theory of neutral and charged excitons in monolaye.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\TXTDCEUI\\Berkelbach et al. - 2013 - Theory of neutral and charged excitons in monolaye.pdf:application/pdf},
}

@article{chernikov_exciton_2014,
	title = {Exciton Binding Energy and Nonhydrogenic Rydberg Series in Monolayer {WS}$_{\textrm{2}}$},
	volume = {113},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.113.076802},
	doi = {10.1103/PhysRevLett.113.076802},
	pages = {076802},
	number = {7},
	journal = {Physical Review Letters},
	shortjournal = {Phys. Rev. Lett.},
	author = {Chernikov, Alexey and Berkelbach, Timothy C. and Hill, Heather M. and Rigosi, Albert and Li, Yilei and Aslan, Burak and Reichman, David R. and Hybertsen, Mark S. and Heinz, Tony F.},
	urldate = {2023-08-31},
	date = {2014-08-13},
	langid = {english},
	file = {Chernikov et al. - 2014 - Exciton Binding Energy and Nonhydrogenic Rydberg S.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\MLD86MT8\\Chernikov et al. - 2014 - Exciton Binding Energy and Nonhydrogenic Rydberg S.pdf:application/pdf},
}

@article{novoselov_electric_2004,
	title = {Electric Field Effect in Atomically Thin Carbon Films},
	volume = {306},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1102896},
	doi = {10.1126/science.1102896},
	abstract = {We describe monocrystalline graphitic films, which are a few atoms thick but are nonetheless stable under ambient conditions, metallic, and of remarkably high quality. The films are found to be a two-dimensional semimetal with a tiny overlap between valence and conductance bands, and they exhibit a strong ambipolar electric field effect such that electrons and holes in concentrations up to 10
              13
              per square centimeter and with room-temperature mobilities of ∼10,000 square centimeters per volt-second can be induced by applying gate voltage.},
	pages = {666--669},
	number = {5696},
	journal = {Science},
	shortjournal = {Science},
	author = {Novoselov, K. S. and Geim, A. K. and Morozov, S. V. and Jiang, D. and Zhang, Y. and Dubonos, S. V. and Grigorieva, I. V. and Firsov, A. A.},
	urldate = {2023-08-31},
	date = {2004-10-22},
	langid = {english},
	file = {Novoselov et al. - 2004 - Electric Field Effect in Atomically Thin Carbon Fi.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\PNL3495N\\Novoselov et al. - 2004 - Electric Field Effect in Atomically Thin Carbon Fi.pdf:application/pdf},
}

@article{chernikov_supplemental_nodate,
	title = {Supplemental Material Non-hydrogenic Rydberg Series and Exciton Binding Energy in Monolayer {WS}2},
	author = {Chernikov, Alexey and Berkelbach, Timothy C and Hill, Heather M and Rigosi, Albert and Li, Yilei and Aslan, Özgur B and Reichman, David R and Hybertsen, Mark S and Heinz, Tony F},
	langid = {english},
	file = {Chernikov et al. - Supplemental Material Non-hydrogenic Rydberg Serie.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\76MGQU9K\\Chernikov et al. - Supplemental Material Non-hydrogenic Rydberg Serie.pdf:application/pdf},
}

@article{van_tuan_coulomb_2018,
	title = {Coulomb interaction in monolayer transition-metal dichalcogenides},
	volume = {98},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.98.125308},
	doi = {10.1103/PhysRevB.98.125308},
	pages = {125308},
	number = {12},
	journal = {Physical Review B},
	shortjournal = {Phys. Rev. B},
	author = {Van Tuan, Dinh and Yang, Min and Dery, Hanan},
	urldate = {2023-08-31},
	date = {2018-09-27},
	langid = {english},
	file = {Van Tuan et al. - 2018 - Coulomb interaction in monolayer transition-metal .pdf:C\:\\Users\\ahonet\\Zotero\\storage\\857MWUFP\\Van Tuan et al. - 2018 - Coulomb interaction in monolayer transition-metal .pdf:application/pdf},
}

@article{rytova_screened_1967,
	title = {THE SCREENED POTENTIAL OF A POINT CHARGE IN A THIN FILM},
	volume = {3},
	pages = {30},
	journal = {Moscow University Physics Bulletin},
	author = {Rytova, N. S.},
	year = {1967},
	langid = {english},
}


@article{keldysh_coulomb_1979,
	title = {Coulomb interaction in thin semiconductor and semimetal films.},
	volume = {29},
	pages = {658–-661},
	number = {11},
	journal = {Journal of Experimental and Theoretical Physics},
	author = {Keldysh, L. V.},
	year = {1979},
	langid = {english},
}

@article{goryca_revealing_2019,
	title = {Revealing exciton masses and dielectric properties of monolayer semiconductors with high magnetic fields},
	volume = {10},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-019-12180-y},
	doi = {10.1038/s41467-019-12180-y},
	abstract = {Abstract
            
              In semiconductor physics, many essential optoelectronic material parameters can be experimentally revealed via optical spectroscopy in sufficiently large magnetic fields. For monolayer transition-metal dichalcogenide semiconductors, this field scale is substantial—tens of teslas or more—due to heavy carrier masses and huge exciton binding energies. Here we report absorption spectroscopy of monolayer
              
                
                  \$\$\{\{{\textbackslash}rm\{{MoS}\}\}\}\_\{2\},\{\{{\textbackslash}rm\{{MoSe}\}\}\}\_\{2\},\{\{{\textbackslash}rm\{{MoTe}\}\}\}\_\{2\}\$\$
                  
                    
                      
                        {MoS}
                      
                      
                        2
                      
                    
                    ,
                    
                      
                        {MoSe}
                      
                      
                        2
                      
                    
                    ,
                    
                      
                        {MoTe}
                      
                      
                        2
                      
                    
                  
                
              
              , and
              
                
                  \$\$\{\{{\textbackslash}rm\{{WS}\}\}\}\_\{2\}\$\$
                  
                    
                      
                        {WS}
                      
                      
                        2
                      
                    
                  
                
              
              in very high magnetic fields to 91 T. We follow the diamagnetic shifts and valley Zeeman splittings of not only the exciton’s
              
                
                  \$\$1s\$\$
                  
                    1
                    s
                  
                
              
              ground state but also its excited
              
                
                  \$\$2s,3s,{\textbackslash}ldots ,ns\$\$
                  
                    2
                    s
                    ,
                    3
                    s
                    ,
                    …
                    ,
                    n
                    s
                  
                
              
              Rydberg states. This provides a direct experimental measure of the effective (reduced) exciton masses and dielectric properties. Exciton binding energies, exciton radii, and free-particle bandgaps are also determined. The measured exciton masses are heavier than theoretically predicted, especially for Mo-based monolayers. These results provide essential and quantitative parameters for the rational design of opto-electronic van der Waals heterostructures incorporating 2D semiconductors.},
	pages = {4172},
	number = {1},
	journal = {Nature Communications},
	shortjournal = {Nat Commun},
	author = {Goryca, M. and Li, J. and Stier, A. V. and Taniguchi, T. and Watanabe, K. and Courtade, E. and Shree, S. and Robert, C. and Urbaszek, B. and Marie, X. and Crooker, S. A.},
	urldate = {2023-08-31},
	date = {2019-09-13},
	langid = {english},
	file = {Goryca et al. - 2019 - Revealing exciton masses and dielectric properties.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\U2FYXNPC\\Goryca et al. - 2019 - Revealing exciton masses and dielectric properties.pdf:application/pdf},
}

@article{mohammadzadeh_excitonic_2013,
	title = {Excitonic effects of bilayer graphene: A simple approach},
	volume = {124},
	issn = {00304026},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0030402613006153},
	doi = {10.1016/j.ijleo.2013.04.083},
	shorttitle = {Excitonic effects of bilayer graphene},
	pages = {6126--6131},
	number = {23},
	journal = {Optik},
	shortjournal = {Optik},
	author = {Mohammadzadeh, L. and Shojaei, S. and Ahmadi, E. and Asgari, A.},
	urldate = {2023-08-31},
	date = {2013-12},
	langid = {english},
	file = {Mohammadzadeh et al. - 2013 - Excitonic effects of bilayer graphene A simple ap.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\9XC59ISH\\Mohammadzadeh et al. - 2013 - Excitonic effects of bilayer graphene A simple ap.pdf:application/pdf},
}

@article{dvali_4d_2000,
	title = {4{D} gravity on a brane in 5{D} Minkowski space},
	volume = {485},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0370269300006699},
	doi = {10.1016/S0370-2693(00)00669-9},
	abstract = {We suggest a mechanism by which four-dimensional Newtonian gravity emerges on a 3-brane in 5D Minkowski space with an infinite size extra dimension. The worldvolume theory gives rise to the correct 4D potential at short distances whereas at large distances the potential is that of a 5D theory. We discuss some phenomenological issues in this framework. q 2000 Elsevier Science B.V. All rights reserved.},
	pages = {208--214},
	number = {1},
	journal = {Physics Letters B},
	shortjournal = {Physics Letters B},
	author = {Dvali, Gia and Gabadadze, Gregory and Porrati, Massimo},
	urldate = {2023-08-31},
	date = {2000-07},
	langid = {english},
	file = {Dvali et al. - 2000 - 4D gravity on a brane in 5D Minkowski space.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\XSIDSML5\\Dvali et al. - 2000 - 4D gravity on a brane in 5D Minkowski space.pdf:application/pdf},
}

@article{dvali_quasilocalized_2001,
	title = {({Q}uasi)localized gauge field on a brane: dissipating cosmic radiation to extra dimensions?},
	volume = {497},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0370269300013290},
	doi = {10.1016/S0370-2693(00)01329-0},
	shorttitle = {(Quasi)localized gauge field on a brane},
	abstract = {We propose a mechanism ensuring (quasi)localization of massless gauge ﬁelds on a brane. The mechanism does not rely on {BPS} properties of the brane and can be realized in any theory where charged particles are conﬁned to the world-volume. The localized matter ﬂuctuations induce a gauge kinetic term on the brane. At short distances the resulting propagator for the gauge ﬁeld is identical to the four-dimensional propagator. The gauge theory on the brane is effectively four-dimensional at short distances; it becomes higher-dimensional on very large (cosmic) scales. The brane-bulk system exhibits the phenomenon of “infrared transparency”. As a result, only very low frequency modes can escape into extra dimensions. In this framework the large wavelength cosmic radiation can dissipate in extra space at a rate that may be observable, in principle. We brieﬂy discuss some astrophysical consequences of this scenario.},
	pages = {271--280},
	number = {3},
	journal = {Physics Letters B},
	shortjournal = {Physics Letters B},
	author = {Dvali, Gia and Gabadadze, Gregory and Shifman, M.},
	urldate = {2023-08-31},
	date = {2001-01},
	langid = {english},
	file = {Dvali et al. - 2001 - (Quasi)localized gauge field on a brane dissipati.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\9XU9VD8Y\\Dvali et al. - 2001 - (Quasi)localized gauge field on a brane dissipati.pdf:application/pdf},
}


@article{vaquero_excitons_2020,
	title = {Excitons, trions and Rydberg states in monolayer {MoS}$_{\mathrm{2}}$ revealed by low-temperature photocurrent spectroscopy},
	volume = {3},
	issn = {2399-3650},
	url = {https://www.nature.com/articles/s42005-020-00460-9},
	doi = {10.1038/s42005-020-00460-9},
	abstract = {Abstract
            
              Exciton physics in two-dimensional semiconductors are typically studied by photoluminescence spectroscopy. However, this technique does not allow for direct observation of non-radiating excitonic transitions. Here, we use low-temperature photocurrent spectroscopy as an alternative technique to investigate excitonic transitions in a high-quality monolayer {MoS}
              2
              phototransistor. The resulting spectra presents excitonic peaks with linewidths as low as 8 {meV}. We identify spectral features corresponding to the ground states of neutral excitons (
              
                
                  \$\$\{{\textbackslash}mathrm\{X\}\}\_\{1\{{\textbackslash}mathrm\{s\}\}\}{\textasciicircum}\{{\textbackslash}mathrm\{A\}\}\$\$
                  
                    
                      
                        X
                      
                      
                        1
                        s
                      
                      
                        A
                      
                    
                  
                
              
              and
              
                
                  \$\$\{{\textbackslash}mathrm\{X\}\}\_\{1\{{\textbackslash}mathrm\{s\}\}\}{\textasciicircum}\{{\textbackslash}mathrm\{B\}\}\$\$
                  
                    
                      
                        X
                      
                      
                        1
                        s
                      
                      
                        B
                      
                    
                  
                
              
              ) and charged trions (T
              A
              and T
              B
              ) as well as up to eight additional spectral lines at energies above the
              
                
                  \$\$\{{\textbackslash}mathrm\{X\}\}\_\{1\{{\textbackslash}mathrm\{s\}\}\}{\textasciicircum}\{{\textbackslash}mathrm\{B\}\}\$\$
                  
                    
                      
                        X
                      
                      
                        1
                        s
                      
                      
                        B
                      
                    
                  
                
              
              transition, which we attribute to the Rydberg series of excited states of X
              A
              and X
              B
              . The intensities of the spectral features can be tuned by the gate and drain-source voltages. Using an effective-mass theory for excitons in two-dimensional systems we are able to accurately fit the measured spectral lines and unambiguously associate them with their corresponding Rydberg states.},
	pages = {194},
	number = {1},
	journal = {Communications Physics},
	shortjournal = {Commun Phys},
	author = {Vaquero, Daniel and Clericò, Vito and Salvador-Sánchez, Juan and Martín-Ramos, Adrián and Díaz, Elena and Domínguez-Adame, Francisco and Meziani, Yahya M. and Diez, Enrique and Quereda, Jorge},
	urldate = {2023-09-01},
	date = {2020-10-30},
	langid = {english},
	file = {42005_2020_460_MOESM1_ESM.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\M7ND2CCY\\42005_2020_460_MOESM1_ESM.pdf:application/pdf;Vaquero et al. - 2020 - Excitons, trions and Rydberg states in monolayer M.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\YGMYWSYF\\Vaquero et al. - 2020 - Excitons, trions and Rydberg states in monolayer M.pdf:application/pdf},
}


@article{pulci_strong_2012,
	title = {Strong excitons in novel two-dimensional crystals: Silicane and germanane},
	volume = {98},
	issn = {0295-5075, 1286-4854},
	url = {https://iopscience.iop.org/article/10.1209/0295-5075/98/37004},
	doi = {10.1209/0295-5075/98/37004},
	shorttitle = {Strong excitons in novel two-dimensional crystals},
	abstract = {We show by ﬁrst-principles calculations that, due to depressed screening and enhanced two-dimensional conﬁnement, excitonic resonances with giant oscillator strength appear in hydrogenated Si and Ge layers, which qualitatively and quantitatively diﬀer from those of graphane. Their large exciton binding energies and oscillator strengths make them promising for observation of novel physical eﬀects and application in optoelectronic devices on the nanoscale.},
	pages = {37004},
	number = {3},
	journal = {{EPL} (Europhysics Letters)},
	shortjournal = {{EPL}},
	author = {Pulci, O. and Gori, P. and Marsili, M. and Garbuio, V. and Del Sole, R. and Bechstedt, F.},
	urldate = {2023-09-01},
	date = {2012-05-01},
	langid = {english},
	file = {Pulci et al. - 2012 - Strong excitons in novel two-dimensional crystals.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\NRGTVH4G\\Pulci et al. - 2012 - Strong excitons in novel two-dimensional crystals.pdf:application/pdf},
}

@article{hsu_dielectric_2019,
	title = {Dielectric impact on exciton binding energy and quasiparticle bandgap in monolayer {WS}$_{\textrm{2}}$ and {WSe}$_{\textrm{2}}$},
	volume = {6},
	issn = {2053-1583},
	url = {https://iopscience.iop.org/article/10.1088/2053-1583/ab072a},
	doi = {10.1088/2053-1583/ab072a},
	abstract = {Excitons, bound electron–hole pairs in a 2D plane, dominate the optical properties of monolayer transition metal dichalcogenides ({TMDs}). A large exciton binding energy on the order of 0.5 {eV} was theoretically predicted and experimentally determined recently. These ultrastable excitons thus open an avenue to explore the exciton physics such as Bose–Einstein condensation and superfluidity at room temperature (Kasprzak et al 2006 Nature 443 409; Plumhof et al 2014 Nat. Mater. 13 247; Fogler et al 2014 Nat. Commun. 5 4555; Jiang and John 2014 Sci. Rep. 4 7432). Recent experiments further demonstrated the concept of Coulomb engineering via dielectric environments based on either solutions or few-layer graphene. However, the conducting nature of these dielectrics can lead to quenching of optical transitions. Thus, in order to utilize ‘dielectric tuning’ of the exciton binding energy and quasiparticle band gaps, one must use insulating dielectrics. Here, we investigate the impact of insulating dielectric environments on the exciton binding energy of monolayer {WS}2 and {WSe}2 by exciton Rydberg spectroscopy, in which the dielectric environment is systematically varied from κ  =  1.49 to 3.82. We found that, with increasing κ value, the exciton binding energy and quasiparticle bandgap exhibit significant reductions. Quantitatively, our result follows the prediction of nonlocally-screened Keldysh potential very well. The fitted 2D polarizability, χ2D, agrees rather well with previous density function theory calculations. Their close agreement validates the nonlocally screened Keldysh model which can be used to quantitatively predict the exciton binding energy for monolayer {TMDs} (and possibly other 2D materials) in different dielectric environments. Such a predictive model will play an important role for the design of van der Waals heterostructures and {TMD}-based optoelectronic devices.},
	pages = {025028},
	number = {2},
	journal = {2D Materials},
	shortjournal = {2D Mater.},
	author = {Hsu, Wei-Ting and Quan, Jiamin and Wang, Chun-Yuan and Lu, Li-Syuan and Campbell, Marshall and Chang, Wen-Hao and Li, Lain-Jong and Li, Xiaoqin and Shih, Chih-Kang},
	urldate = {2023-09-01},
	date = {2019-03-07},
	langid = {english},
	file = {Hsu et al. - 2019 - Dielectric impact on exciton binding energy and qu.pdf:C\:\\Users\\ahonet\\Zotero\\storage\\6HIMRNLH\\Hsu et al. - 2019 - Dielectric impact on exciton binding energy and qu.pdf:application/pdf},
}

@phdthesis{honet_master_2019,
  TITLE = {Mécanisme Dvali-Gabadadze-Porrati-Shifman et
électrodynamique quantique à (2+1) dimensions.
Application à un modèle d’exciton dans le
graphène.},
  AUTHOR = {Honet, Antoine},
  SCHOOL = {{Université Libre de Bruxelles (ULB)}},
  YEAR = {2019},
  TYPE = {Theses},
}


@book{gradshteyn_table_2015,
	address = {Waltham, Mass},
	title = {Table of Integrals, Series, and Products. 8th edition},
	publisher = {Academic
Press},
	author = {Gradshteyn, Izrail Solomonovich and Ryzhik, Iosif Moiseevich},
	date = {2015},
	year = {2015},

}

@book{abramowitz_1970,
	title = {Handbook of Mathematical Functions: with Formulas, Graphs, and Mathematical Tables},
	publisher = {National Bureau of Standards },
	author = {Abramowitz, Milton and Stegun, Irene A. },
	date = {1970},
	year = {1970},

}


@article{mcdonald2019electrodynamics,
  title={Electrodynamics in 1 and 2 spatial dimensions},
  author={McDonald, Kirk T},
  journal={unpublished notes},
  year={2019}
}

@article{boito_maxwells_2020,
	title = {On {Maxwell}’s electrodynamics in two spatial dimensions},
	volume = {42},
	copyright = {http://creativecommons.org/licenses/by/4.0/},
	issn = {1806-9126, 1806-1117},
	url = {http://www.scielo.br/scielo.php?script=sci_arttext&pid=S1806-11172020000100444&tlng=en},
	doi = {10.1590/1806-9126-rbef-2019-0323},
	urldate = {2024-12-17},
	journal = {Revista Brasileira de Ensino de Física},
	author = {Boito, D. and Andrade, L. N. S. De and Sousa, G. De and Gama, R. and London, C. Y. M.},
	year = {2020},
	pages = {e20190323},
}

@article{lapidus_classical_1982,
	title = {Classical electrodynamics in a universe with two space dimensions},
	volume = {50},
	issn = {0002-9505, 1943-2909},
	url = {https://pubs.aip.org/ajp/article/50/2/155/1051850/Classical-electrodynamics-in-a-universe-with-two},
	doi = {10.1119/1.12875},
	language = {en},
	number = {2},
	urldate = {2024-12-17},
	journal = {American Journal of Physics},
	author = {Lapidus, I. Richard},
	year = {1982},
	pages = {155--157},
}

@article{nguyen-truong_exciton_2022,
	title = {Exciton binding energy and screening length in two-dimensional semiconductors},
	volume = {105},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.105.L201407},
	doi = {10.1103/PhysRevB.105.L201407},
	language = {en},
	number = {20},
	urldate = {2024-12-17},
	journal = {Physical Review B},
	author = {Nguyen-Truong, Hieu T.},
	year = {2022},
	pages = {L201407},
}

@article{galiautdinov_anisotropic_2019,
	title = {Anisotropic {Keldysh} interaction},
	volume = {383},
	issn = {03759601},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0375960119305870},
	doi = {10.1016/j.physleta.2019.07.002},
	language = {en},
	number = {25},
	urldate = {2024-12-17},
	journal = {Physics Letters A},
	author = {Galiautdinov, Andrei},
	year = {2019},
	pages = {3167--3174},
}

@article{kirichenko_influence_2021,
	title = {The influence of {Coulomb} interaction screening on the excitons in disordered two-dimensional insulators},
	volume = {11},
	issn = {2045-2322},
	url = {https://www.nature.com/articles/s41598-021-91414-w},
	doi = {10.1038/s41598-021-91414-w},
	language = {en},
	number = {1},
	urldate = {2024-12-17},
	journal = {Scientific Reports},
	author = {Kirichenko, E. V. and Stephanovich, V. A.},
	year = {2021},
	pages = {11956},
}

@article{Henriques:21,
author = {J. C. G. Henriques and M. F. C. Martins Quintela and N. M. R. Peres},
journal = {J. Opt. Soc. Am. B},
keywords = {Femtosecond lasers; Laser pumping; Optical computing; Optical elements; Optical properties; Photon counting},
number = {7},
pages = {2065--2074},
publisher = {Optica Publishing Group},
title = {Theoretical model of the polarizability due to transitions between exciton states in transition metal dichalcogenides: application to {WSe}$_{\mathrm{2}}$},
volume = {38},
year = {2021},
url = {https://opg.optica.org/josab/abstract.cfm?URI=josab-38-7-2065},
doi = {10.1364/JOSAB.421279},

}

@article{henriques_analytical_2020,
	title = {Analytical quantitative semiclassical approach to the {Lo} {Surdo}–{Stark} effect and ionization in two-dimensional excitons},
	volume = {102},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.102.035402},
	doi = {10.1103/PhysRevB.102.035402},
	language = {en},
	number = {3},
	urldate = {2024-12-17},
	journal = {Physical Review B},
	author = {Henriques, J. C. G. and Kamban, Høgni C. and Pedersen, Thomas G. and Peres, N. M. R.},
	year = {2020},
	pages = {035402},
}

@article{zaslow_two-dimensional_1967,
	title = {Two-{Dimensional} {Analog} to the {Hydrogen} {Atom}},
	volume = {35},
	issn = {0002-9505, 1943-2909},
	url = {https://pubs.aip.org/ajp/article/35/12/1118/1047824/Two-Dimensional-Analog-to-the-Hydrogen-Atom},
	doi = {10.1119/1.1973790},
	abstract = {The Schrödinger equation is applied to a two-dimensional problem of two mass points, one with the charge and mass of an electron and the other with the charge and mass of a proton. Solution exists in closed form, and the result is compared with that for a three-dimensional hydrogen atom.},
	language = {en},
	number = {12},
	urldate = {2024-12-18},
	journal = {American Journal of Physics},
	author = {Zaslow, B. and Zandler, Melvin E.},
	year = {1967},
	pages = {1118--1119},
}

@book{lowe_quantum_2006,
	address = {Amsterdam},
	edition = {3rd ed},
	title = {Quantum chemistry},
	isbn = {978-0-12-457551-6},
	language = {eng},
	publisher = {Elsevier},
	author = {Lowe, John P. and Peterson, Kirk A.},
	year = {2006},
}

@book{le_bellac_phenomenes_2002,
	address = {Les Ulis, France},
	series = {Savoirs actuels. {Physique}},
	title = {Des phénomènes critiques aux champs de jauge: une introduction aux méthodes et aux applications de la théorie quantique des champs},
	isbn = {978-2-86883-359-4 978-2-7598-0284-5},
	shorttitle = {Des phénomènes critiques aux champs de jauge},
	language = {fr},
	publisher = {EDP Sciences},
	author = {Le Bellac, Michel},
	year = {2002},
	file = {Le Bellac - 2002 - Des phénomènes critiques aux champs de jauge une .pdf:C\:\\Users\\Antoine\\Zotero\\storage\\LYBICTEW\\Le Bellac - 2002 - Des phénomènes critiques aux champs de jauge une .pdf:application/pdf},
}

@book{kittel_introduction_nodate,
	address = {Hoboken, NJ},
	edition = {8. ed., [repr.]},
	title = {Introduction to solid state physics},
	isbn = {978-0-471-41526-8},
	language = {en},
	publisher = {Wiley},
	author = {Kittel, Charles},
    year = {2004},
	file = {Kittel - Introduction to solid state physics.pdf:C\:\\Users\\Antoine\\Zotero\\storage\\CRIV6MFR\\Kittel - Introduction to solid state physics.pdf:application/pdf},
}

@book{cohen-tannoudji_quantum_2020,
	address = {Weinheim},
	edition = {Second edition},
	title = {Quantum mechanics. {Volume} 1: {Basic} concepts, tools, and applications},
	isbn = {978-3-527-34553-3},
	shorttitle = {Quantum mechanics. {Volume} 1},
	language = {en},
	publisher = {Wiley-VCH Verlag GmbH \& Co. KGaA},
	author = {Cohen-Tannoudji, Claude and Diu, Bernard and Laloë, Franck},
	translator = {Reid Hemley, Susan and Ostrowsky, Nicole and Ostrowsky, Dan},
	year = {2020},
	file = {Cohen-Tannoudji et al. - 2020 - Quantum mechanics. Volume 1 Basic concepts, tools.pdf:C\:\\Users\\Antoine\\Zotero\\storage\\CNL2YSU8\\Cohen-Tannoudji et al. - 2020 - Quantum mechanics. Volume 1 Basic concepts, tools.pdf:application/pdf},
}

@article{rubakov_we_1983,
	title = {Do we live inside a domain wall?},
	volume = {125},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0370269383912534},
	doi = {10.1016/0370-2693(83)91253-4},
	language = {en},
	number = {2-3},
	urldate = {2025-03-05},
	journal = {Physics Letters B},
	author = {Rubakov, V.A. and Shaposhnikov, M.E.},
	month = may,
	year = {1983},
	pages = {136--138},
}

@article{hughes_supermembranes_1986,
	title = {Supermembranes},
	volume = {180},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {03702693},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0370269386912049},
	doi = {10.1016/0370-2693(86)91204-9},
	language = {en},
	number = {4},
	urldate = {2025-03-05},
	journal = {Physics Letters B},
	author = {Hughes, James and Liu, Jun and Polchinski, Joseph},
	month = nov,
	year = {1986},
	pages = {370--374},
}

@article{lukas_universe_1999,
	title = {Universe as a domain wall},
	volume = {59},
	copyright = {http://link.aps.org/licenses/aps-default-license},
	issn = {0556-2821, 1089-4918},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.59.086001},
	doi = {10.1103/PhysRevD.59.086001},
	language = {en},
	number = {8},
	urldate = {2025-03-05},
	journal = {Phys. Rev. D},
	author = {Lukas, André and Ovrut, Burt A. and Stelle, K. S. and Waldram, Daniel},
	month = mar,
	year = {1999},
	pages = {086001},
	file = {Full Text:C\:\\Users\\Administrator\\Zotero\\storage\\VGH28W8D\\Lukas et al. - 1999 - Universe as a domain wall.pdf:application/pdf},
}

@article{davies_standard_2008,
	title = {Standard model on a domain-wall brane?},
	volume = {77},
	copyright = {http://link.aps.org/licenses/aps-default-license},
	issn = {1550-7998, 1550-2368},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.77.124038},
	doi = {10.1103/PhysRevD.77.124038},
	language = {en},
	number = {12},
	urldate = {2025-03-05},
	journal = {Phys. Rev. D},
	author = {Davies, Rhys and George, Damien P. and Volkas, Raymond R.},
	month = jun,
	year = {2008},
	pages = {124038},
	file = {Submitted Version:C\:\\Users\\Administrator\\Zotero\\storage\\5E3353F4\\Davies et al. - 2008 - Standard model on a domain-wall brane.pdf:application/pdf},
}

@article{maartens_brane-world_2004,
	title = {Brane-{World} {Gravity}},
	volume = {7},
	issn = {2367-3613, 1433-8351},
	url = {http://link.springer.com/10.12942/lrr-2004-7},
	doi = {10.12942/lrr-2004-7},
	language = {en},
	number = {1},
	urldate = {2025-03-05},
	journal = {Living Rev. Relativ.},
	author = {Maartens, Roy},
	month = dec,
	year = {2004},
	pages = {7},
	file = {Full Text:C\:\\Users\\Administrator\\Zotero\\storage\\5PK38XX5\\Maartens - 2004 - Brane-World Gravity.pdf:application/pdf},
}

@article{brax_brane_2004,
	title = {Brane world cosmology},
	volume = {67},
	issn = {0034-4885, 1361-6633},
	url = {https://iopscience.iop.org/article/10.1088/0034-4885/67/12/R02},
	doi = {10.1088/0034-4885/67/12/R02},
	number = {12},
	urldate = {2025-03-05},
	journal = {Rep. Prog. Phys.},
	author = {Brax, Philippe and Bruck, Carsten Van De and Davis, Anne-Christine},
	month = dec,
	year = {2004},
	pages = {2183--2231},
}

@article{koivisto_dark_2014,
	title = {Dark {D}-brane cosmology},
	volume = {2014},
	copyright = {http://iopscience.iop.org/info/page/text-and-data-mining},
	issn = {1475-7516},
	url = {https://iopscience.iop.org/article/10.1088/1475-7516/2014/06/036},
	doi = {10.1088/1475-7516/2014/06/036},
	number = {06},
	urldate = {2025-03-05},
	journal = {J. Cosmol. Astropart. Phys.},
	author = {Koivisto, Tomi and Wills, Danielle and Zavala, Ivonne},
	month = jun,
	year = {2014},
	pages = {036--036},
	file = {Full Text:C\:\\Users\\Administrator\\Zotero\\storage\\94VNBYAA\\Koivisto et al. - 2014 - Dark D-brane cosmology.pdf:application/pdf},
}

@article{arkani-hamed_manyfold_2000,
	title = {Manyfold universe},
	volume = {2000},
	issn = {1029-8479},
	url = {http://stacks.iop.org/1126-6708/2000/i=12/a=010?key=crossref.7ef557d719d14620a9256c1f1f4b7d40},
	doi = {10.1088/1126-6708/2000/12/010},
	number = {12},
	urldate = {2025-03-05},
	journal = {J. High Energy Phys.},
	author = {Arkani-Hamed, Nima and Dimopoulos, Savas and Kaloper, Nemanja and Dvali, Gia},
	month = dec,
	year = {2000},
	pages = {010--010},
	file = {Submitted Version:C\:\\Users\\Administrator\\Zotero\\storage\\KDAC3NMP\\Arkani-Hamed et al. - 2000 - Manyfold universe.pdf:application/pdf},
}

@article{bhattacharya_cosmological_2018,
	title = {Cosmological screening and the phantom braneworld model},
	volume = {78},
	issn = {1434-6044, 1434-6052},
	url = {http://link.springer.com/10.1140/epjc/s10052-018-6119-z},
	doi = {10.1140/epjc/s10052-018-6119-z},
	language = {en},
	number = {8},
	urldate = {2025-03-05},
	journal = {Eur. Phys. J. C},
	author = {Bhattacharya, Sourav and Kousvos, Stefanos R. and Romanopoulos, Stylianos and Tomaras, Theodore N.},
	month = aug,
	year = {2018},
	pages = {637},
	file = {Full Text:C\:\\Users\\Administrator\\Zotero\\storage\\C57VZENB\\Bhattacharya et al. - 2018 - Cosmological screening and the phantom braneworld model.pdf:application/pdf},
}

@article{bhattacharya_constraining_2017,
	title = {Constraining the phantom braneworld model from cosmic structure sizes},
	volume = {96},
	copyright = {https://link.aps.org/licenses/aps-default-license},
	issn = {2470-0010, 2470-0029},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.96.104006},
	doi = {10.1103/PhysRevD.96.104006},
	language = {en},
	number = {10},
	urldate = {2025-03-05},
	journal = {Phys. Rev. D},
	author = {Bhattacharya, Sourav and Kousvos, Stefanos R.},
	month = nov,
	year = {2017},
	pages = {104006},
	file = {Submitted Version:C\:\\Users\\Administrator\\Zotero\\storage\\XD8TTJYV\\Bhattacharya and Kousvos - 2017 - Constraining the phantom braneworld model from cosmic structure sizes.pdf:application/pdf},
}

